Anomalous Diffusion in a Bench-Scale Pulsed Fluidized Bed

We present our analysis on micro-rheology of a bench-scale pulsed fluidized bed, which represents a weakly confined system. Non-linear gas-particle and particle-particle interactions resulting from pulsed flow are associated with harmonic and sub-harmonic modes. While periodic structured bubble patterns are observed at the meso-scale, particle-scale measurements reveal anomolous diffusion in the driven granular medium. We use single-particle tracks to analyze ergodicity and ageing properties at two pulsing frequencies having remarkably different meso-scale features. The scaling of ensemble-averaged mean squared displacement is not unique. The distribution of time-averaged mean squared displacements is non-Gaussian, asymmetric and has a finite trivial contribution from particles in crowded quasi-static surroundings. Results indicate weak ergodicity breaking which along with ageing characterize the non-stationary and out-of-equilibrium dynamics.

==> sec1.tex <==
Multiphase flows exhibit a range of spatio-temporal scales arising from complex non-linear dynamics \cite{Zhao2003,Blomgren2007,Fullmer2017,AV2017CES,AV2019,AV2020}. Fluidization is a notable example, in which particles are suspended by an incoming stream of fluid, whereby they exhibit fluid-like behavior. Travelling kinematic waves in the form of bubbles representing spatial inhomogeneities in solids concentration are common in such systems. In particular, pulsed fluidized beds (PFBs) are characterized by a repeatable bubbling pattern resulting from dynamical structuring and suppression of chaos compared to fluidized beds having a non-perturbed inflow. PFBs have shown improved hydrodynamics by reducing or eliminating channeling or clumping of particles, and enhanced heat and mass transfer properties while being non-intrusive. Studies in the past have primarily reported on the meso-scale and macro-scale observations in PFBs \cite{Pence98,Coppens2003,Coppens2012,Wu2017,Coppens2018,Higham2020}. Persistent interactions between dynamical modes are present at different scales, and particle-level description is pivotal in elucidating some of the observed features. Particles evolve depending on a number of factors including external forcing, momentum exchange with the carrier-phase and neighbors, material properties and confines of the system. It is intuitive that in the presence of localized features, different particles have different driving mechanisms. For instance, particles in the vicinity of bubble wakes experience a greater acceleration compared to those near the distributor or other quasi-static zones. We use the term quasi-two-dimensional (quasi-2D) to describe PFB used in this study, since the extent in the depth-wise direction is comparable to the size of bubbles, further verified by high-speed videos which reveal their span.

Previous studies \cite{vanNoije98,Barrat02,BenNaim05,Moka05,AV2017} have examined velocity fluctuations and reported deviations from ideal Brownian motion. The simplistic assumption of Maxwellian distribution breaks down quite easily in multi-particle systems, and results in anomalous diffusion described by,

\begin{equation}
    \langle x^{2}(\Delta) \rangle \sim \Delta^{\gamma}
\end{equation}

\noindent The process is sub-diffusive for $\gamma$ < 1 and super-diffusive for $\gamma$ > 1, both of which are observed in nature and engineering applications \cite{Solomon1993,Wong2004,Xie2008,Mattsson2009,Bronstein2009,Krapf2011,Kneller2011,Palombo2013}, while $\gamma$ = 1 describes normal Brownian diffusion. There also exist possible flow scenarios which cannot be described by a unique value of $\gamma$ and involve transition of regimes discussed above. Different sources of anomalous diffusion have been studied in the past which include Continuous-Time Random Walk (CTRW), Fractional Brownian Motion (FBM) and the motion governed by Fractional Langevin Equation (FLE), Scaled Brownian Motion (SBM), Transport on a Fractal Support, and Heterogeneous Diffusion Process (HDP). Previous analyses also include combining these parent processes such as CTRW-FLE \cite{Metzler2014-PRX} and SBM-HDP \cite{Metzler2015}, the latter was termed Generalized Diffusion Process (GDP), where diffusivity varies in space and time as follows,

\begin{equation}
\label{eq:GDP}
    D(x,t) \sim (1+\beta)D_{0} |x|^{\alpha} t^{\beta}
\end{equation}

\noindent The above equation combines spatial and temporal dependence from the underlying HDP and SBM respectively. GDP is sub-diffusive ($\gamma < 1$) when $\alpha > 2 \beta + 4$, and super-diffusive ($\gamma > 1$) otherwise. Based on the physics of PFB as explained in our previous study \cite{Higham2020}, we hypothesize the system hosts a combination of parent processes discussed above, as will be shown in the remainder of this article. We also study the effect of ageing i.e., the time lapsed after initializing an experiment. It must be noted that PFB does not represent confinement in a strict sense. Boundaries or walls are present which reflect particles after inelastic collisions in the lateral direction, while the streamwise transport is governed by balance between drag exerted by the carrier-phase and gravity. Hence, we use the term weak confinement to describe PFB.

%We can hence expect a non-uniform position dependent diffusion often categorized under heterogeneous diffusion process (HDP). In the past, HDPs have been shown to exhibit anomalous diffusion and non-ergodic dynamics (\textcolor{red}{Reference of Meltzer and co-workers}) which is expected to be the case in PFBs as well.

%In this study, we analyze micro-rheology of a small-scale PFB.

%particle-particle or particle-carrier phase interactions. Standing wave patterns and kinks have been observed in vertically vibrated granular beds (\textcolor{red}{References for vibrating bed}). Systems also exhibit meso-scale structures such as clusters and bubbles (\textcolor{red}{References for clustering}) by interacting with the gas phase. Occurrence of such structures may lead to anomalous diffusion prevalent in several engineering applications and biological systems \cite{Solomon1993,Palombo2013}. 

%Anomalous diffusion also affects the particle velocity distribution function (VDF). The non-equilibrium VDFs in forced systems quantify the cascade of energy. Besides, the tail population may have a significant effect on the heat and mass transfer characteristics for reacting systems. Even from a modeling perspective, it is critical to know the representative form of VDF. Kinetic theory (KT) formulation provide an elegant framework for modeling granular flows. The closure relations are obtained from the moments of VDFs and the naive approach is to assume a Gaussian form. Deviations from Gaussian distribution have also been considered in the past. A stretched exponential VDF of the form $P(c) \sim e^{-\alpha |c|^\beta}$ was considered by van Noije and Ernst \cite{vanNoije98} and Barrat et al. \cite{Barrat02}. Ben-Naim and Krapivsky \cite{BenNaim02} use a power-law to describe the tail, $P(c) \sim |c|^{-\gamma}$ which has also been reported in experiments \cite{Moka05} and numerical simulations \cite{BenNaim05}. 

%In this letter, we report particle statistics in a quasi-2D pulsed fluidized bed (PFB) system. PFBs are characterized by a wide range of spatio-temporal scales and exhibit periodic periodic bubbling pattern, and was first demonstrated by Coppens and his co-workers \textcolor{red}{Coppens}. Very limited experimental efforts related to PFBs exist currently and our study is aimed at providing further details regarding the particle-scale dynamics. The experiments were designed to record particle tracks for a significant duration $\sim 40s$. The VDFs have a symmetric non-Maxwellian distribution reflecting the Levy-flight process associated with the bubble movement inside the bed. The measured diffusion coefficient is time dependent and indicates transition from super-diffusive to sub-diffusive regime. The Fourier transform of the velocity fluctuations reveals characteristic frequencies in the bubbling system. 

==> sec2.tex <==
The experiments were performed using a quasi-2D geometry shown in Figure ~\ref{fig:Schematic}. The bed was filled with 18$g$ glass particles having a Sauter mean diameter of 394$\mu m$ and a density of 2.5$g/cc$, classified under Geldart Group B \cite{Geldart1973}. Flow rate at the inlet is pulsed in the form of a sine wave,

\begin{equation}
    Q(t) = \mathrm{A + B\: sin} (2 \mathrm{\pi f} t)
\end{equation}

\noindent where, the base flow rate A = 2.6$l/min$ is set such that the velocity is higher than the minimum fluidization velocity, $U_{mf}$ which denotes the minimum velocity required to support the weight of solids. Details regarding the measurement of $U_{mf}$ can be found in \citet{AV-TRS2020}. The amplitude B is set to 2.1$l/min$. In this study, we analyze the dynamics of particulate phase under two pulsing frequencies, f = 4$hz$ and 6$hz$. A fractal distributor was 3-D printed (Figure ~\ref{fig:Schematic}) using a high-precision ultraviolet curing printer. High-speed videos were captured at 300$hz$ over a duration of 20$s$ using a 120$mm$ Nikon lens and Fastex IL5L sensor, and the unit was back-lit using an LED light source. The resulting spatial resolution was 0.71$mm$ X 0.71$mm$. Glass particles were tracked using an in-house code, PTVResearch \cite{Fullmer2020} and optical distortions were removed using a calibrated grid and polynomial de-warping technique \cite{Higham2019}. Individual tracks were determined by Optical Flow Equations, and the outliers were detected based on proper orthogonal decomposition technique \cite{Higham2016}. Further details regarding the experiments have been avoided for the sake of brevity, and can be found in \citet{Higham2020}.

%The bubbling pattern however is a function of the the mean velocity, and the amplitude and frequency of oscillations. In this study, the inlet mean velocity and the amplitude are fixed, and the gas flow rate is pulsed at 4 hz and 6 hz. The bubble configuration transitions from an alternating 1-1 pattern at 4 hz to a 1-2-1 pattern at 6 hz as shown in Figure (\textcolor{red}{bubble pattern}). The details regarding the image processing are as follows: (\textcolor{red}{Jonny's input on image processing}). 

\begin{figure}[!htpb]
\begin{center}
\includegraphics[width=0.9\linewidth]{Schematic.png}
\end{center}
\caption{Schematic of the PFB set-up used in this study. The zoomed-in image and its inset show the frontal view of fractal distributor and its rough sketch (not drawn to scale).}
\label{fig:Schematic}
\end{figure}

Images reveal meso-scale response of the system to pulsing conditions (Figure ~\ref{fig:Schematic2}). At f = 4$hz$, bubbles alternate from wall to wall, while the pattern changes to a bubble at the center and two simultaneous bubbles along the wall at 6$hz$. There is an active interaction between harmonic and sub-harmonic modes associated with each configuration as explained in our previous study \cite{Higham2020}. Force chains are repeatedly formed and broken depending on f, and the rate at which this occurs determines the bubbling pattern having a characteristic wavelength $\lambda$. $\lambda$ representative of bubble size appears to drop while changing f from 4$hz$ to 6$hz$, and the bubbles are shifted by $\lambda/2$ between successive cycles.

\begin{figure}[!htpb]
\begin{center}
\includegraphics[width=\linewidth]{Pattern.png}
\end{center}
\caption{Bubbling pattern in the PFB at f = 4$hz$ (top) and 6$hz$ (bottom).}
\label{fig:Schematic2}
\end{figure}

==> sec3.tex <==
Arbitrarily chosen particle tracks are shown in Figure ~\ref{fig:trajectory} indicating a non-uniform diffusion coefficient in the PFB. Trajectories evolve depending on the initial location as well as appear to have a temporal dependence. We also notice a few tracks which are transported over much shorter distances compared to the rest. Even if a single particle track is considered, depending on the time instance, the motion is altered significantly. If we were to describe using meso-scale features, particles in the wake of bubbles are associated with longer steps, while they undergo much shorter displacements away from the vicinity of such kinematic waves. Also, the motion is confined by walls in the lateral direction, while the balance between gravity and inter-phase drag determines the streamwise transport. Particle trajectories are influenced by carrier-phase depending on their location, a mechanism neither trivial nor explicitly modeled in most of the studies describing anomalous diffusion. In the framework of kinetic theory, the effect due to drag was recently included in the generalized Langevin equation, \cite{garzo2012} and further efforts are required to substantiate this approach.

%Histograms of normalized step increments show a symmetric distribution in the transverse direction which lacks external forcing. There is a noticeable asymmetry in the streamwise direction ~\ref{fig:histogram} caused by the counteracting gravity and drag force exerted by the carrier-phase. A prominent cusp at $\Delta_{i} = 0$, and over-populated tails are observed, which are further suggestive of non-Brownian diffusion. 

%Step increments of two randomly chosen particles in the cartesian coordinates are shown in Figures ~\ref{fig:trajectory}. This is the first indicator of anomalous diffusion in the PFB associated with a non-uniform diffusion coefficient, as the two traces are completely different for each case. Histograms of normalized step increments show a symmetric distribution in the transverse direction which lacks external forcing. There is a noticeable asymmetry in the streamwise direction ~\ref{fig:histogram} caused by the counteracting gravity and drag force exerted by the carrier-phase. A prominent cusp at $\Delta_{i} = 0$, and over-populated tails are observed, which are further suggestive of non-Brownian diffusion. 

\begin{figure}[!htpb]
\begin{center}
\includegraphics[width=\linewidth]{Trajectories-4hz-6hz.png}
\end{center}
\caption{Sample trajectories at f = 4$hz$ (left) and 6$hz$ (right).}
\label{fig:trajectory}
\end{figure}

%\begin{figure}[!htpb]
%\begin{center}
%\includegraphics[width=0.8\linewidth]{TimeSeries-4hz.png}
%\end{center}
%\caption{Time trace of step increments at f = 4hz in lateral (top) and streamwise (bottom) directions. P1 and P2 are randomly chosen time traces.}
%\label{fig:trajectory1}
%\end{figure}

%\begin{figure}[!htpb]
%\begin{center}
%\includegraphics[width=0.8\linewidth]{TimeSeries-6hz.png}
%\end{center}
%\caption{Time trace of step increments at f = 6hz in lateral (top) and streamwise (bottom) directions. P1 and P2 are randomly chosen time traces.}
%\label{fig:trajectory2}
%\end{figure}

%\begin{figure}[!htpb]
%\begin{center}
%\begin{subfigure}{0.7\linewidth}
%    \includegraphics[width=\linewidth]{histogram-dx.png}
%\end{subfigure}
%\begin{subfigure}{0.7\linewidth}
%    \includegraphics[width=\linewidth]{histogram-dy.png}
%\end{subfigure}
%\end{center}
%\caption{Histogram of step increments for f=4hz and 6hz in the lateral (top) and streamwise (bottom) directions. The steps are normalized using standard deviations, $\sqrt{2 \sigma_{\Delta_{x}^{2}}}$ and $\sqrt{2 \sigma_{\Delta_{y}^{2}}}$.}
%\label{fig:histogram}
%\end{figure}

Next, we look at the autocorrelation, $\mathrm{A}$ between displacements or step increments in the cartesian directions. We use the following definition,

\begin{equation}
\label{eq:ACF}
    \mathrm{A}(\Delta) = \frac{\mathbf{E}\big[x_{i}(t) x_{i}(t+\Delta)\big]}{\sqrt{\mathbf{Var}\big[x_{i}(t)\big] \mathbf{Var}\big[x_{i}(t+\Delta)\big]}}
\end{equation}

\noindent This is ensemble-averaged to obtain $\mathrm{\langle A \rangle}$ shown in Figure ~\ref{fig:ACF}. We notice dominant harmonic and sub-harmonic modes at both the pulsing frequencies. The decay of $\mathrm{\langle A \rangle}$ for the lateral transport of particles is predominant compared to their streamwise component at f=4$hz$, while the behavior is similar in the two coordinate directions at f=6$hz$. This is associated with redistribution of energy between harmonic and sub-harmonic modes as explained using Proper Orthogonal Decomposition \cite{Higham2020}. The long-range correlation (memory effects) observed in the collective behavior of particles follows the idea of Kac \cite{Kac1956}, wherein determinism evolves in multi-particle systems governed by stochastic differential equations, which in this case appear to vary depending on the spatial location of particles.

\begin{figure}[!htpb]
\begin{center}
\includegraphics[width=\linewidth]{ACF-4hz-6hz.png}
\end{center}
\caption{ACF plots of x and y displacement for f = 4$hz$ (top) and 6$hz$ (bottom).}
\label{fig:ACF}
\end{figure} 

~\noindent We then examine the behavior of mean-squared displacement (MSD), typically used to study diffusion processes. Ergodicity in PFB is yet to be confirmed, and we use two different measures of MSD. First, is the ensemble averaged MSD given by,

\begin{equation}
\label{eq:MSD1}
    \langle \mathrm{x^{2}}(\Delta) \rangle = \frac{1}{N} \sum_{i=1}^{N} |\mathrm{x_{i}}(\Delta) - \mathrm{x_{i}}(0)|^{2}
\end{equation}

\noindent Second, is the time-averaged MSD given by,

\begin{equation}
\label{eq:MSD2}
    \langle \mathrm{\overline{\delta^{2}(\Delta)}} \rangle = \frac{1}{\mathrm{T}-\Delta} \int_{0}^{\mathrm{T}-\Delta} \langle |x_{i}(t+\Delta) - x_{i}(t)|^{2} \rangle dt
\end{equation}

\noindent which involves both time-averaging and ensemble-averaging operators. $\Delta$ and T refer to lag time and total measurement time. Figure ~\ref{fig:MSD} represents MSDs evaluated from particle tracks. Plots of $\langle \mathrm{x^{2}} \rangle$ confirm that a single value of $\gamma$ cannot be used to describe the anomalous diffusion process. Besides, we notice difference in scaling between $\langle \mathrm{x^{2}} \rangle$ and $\langle \mathrm{\overline{\delta^{2}}} \rangle$ indicating weak non-ergodicity \cite{Bel2005,Metzler2007,Sokolov2012,Metzler2014}. This eliminates the possibility of diffusion in PFB describing transport on a fractal support, which is an ergodic process. We also observe that $\langle \mathrm{\overline{\delta^{2}}} \rangle$ approaches a plateau as $\Delta \to T$ ($\langle \mathrm{x^{2}} \rangle \sim \Delta^{0}$) moreso for f=6$hz$, reported previously for confined GDPs and SBMs by Metzler et al. \cite{Metzler2014,Metzler2015}. This is in contrast to purely sub-diffusive CTRWs, where plateaus are not present for time-averaged MSD. $\langle \mathrm{x^{2}} \rangle$ and $\langle \mathrm{\overline{\delta^{2}}} \rangle$ show the same limiting behavior at $\Delta/T \to 0$ and $\Delta/T \to 1$. The latter is apparent from Equation ~\ref{eq:MSD2}, which has a singularity in the limit of $\Delta \to T$, thus placing the constraint, $\langle \mathrm{x^{2}} \rangle = \langle \mathrm{\overline{\delta^{2}}} \rangle$. Also, $\langle \mathrm{\overline{\delta^{2}}} \rangle$ varies $\propto \Delta^{1}$ over an appreciable time frame for both the values of f, previously observed for sub- and super-difussive unconfined HDPs \cite{Metzler2014}. This might lead to a false impression of normal Brownian motion unless properly addressed using complementary statistical measures.

%The slope of $\langle \mathrm{x^{2}}$ transitions to $\Delta^{0}$ earlier at f=6 $\text{Hz}$ suggesting particles diffuse to the boundaries faster compared to f=4 $\text{Hz}$.

\begin{figure}[!htpb]
\begin{center}
\begin{subfigure}{0.8\linewidth}
    \includegraphics[width=\linewidth]{MSD-EA-TA-4hz.png}
\end{subfigure}
\begin{subfigure}{0.8\linewidth}
    \includegraphics[width=\linewidth]{MSD-EA-TA-6hz.png}
\end{subfigure}
\end{center}
\caption{MSD from experiments at f = 4 $hz$ (top) and 6 $hz$ (bottom). Dashed lines represent $\Delta^1$ sacling.}
\label{fig:MSD}
\end{figure}

To elucidate non-ergodic dynamics in PFB, we define ergodicity breaking parameter (EB) as,

\begin{equation}
\label{eq:EB}
\mathrm{EB(\Delta)} = \frac{\langle \overline{\delta^{2}(\Delta)}^2 \rangle}{\langle \mathrm{\overline{\delta^{2}(\Delta)}} \rangle^2} - 1
\end{equation}

\noindent $\mathrm{EB}$ quantifies dispersion of time-averaged MSDs, $\mathrm{\overline{\delta^{2}}}$. We use variation in $\mathrm{EB}$ as a function of measurement time, T to describe non-ergodicity, where $\Delta$ = 0.017$s$ is chosen for demonstration. $\mathrm{EB}$ for a Brownian motion follows $\lim_{\Delta/T \to 0} \mathrm{EB_{BM}(\Delta)} = \frac{4}{3}\frac{\Delta}{T}$, indicated by the curve $\propto \mathrm{T}^{-1}$ in Figure ~\ref{fig:EB}. We observe a more gradual change in EB leading to an asymptotic finite value in the limit of T$\to \infty$. This has been reported previously for anomalous stochastic processes governed by HDPs and CTRWs \cite{Metzler2015ChemPhys}. To further investigate the nature of ergodicity breaking, we use alternative ergodic parameter, $\mathcal{EB}$ following the definition of \citet{Metzler2013} given by,

\begin{equation}
\label{eq:EB2}
\mathrm{\mathcal{EB}(\Delta)} = \frac{ \langle \mathrm{\overline{\delta^{2}(\Delta)}} \rangle}{\langle \mathrm{x^{2}}(\Delta) \rangle}
\end{equation}

\noindent A necessary condition for ergodicity is $\mathcal{EB}=1$, while a sufficient condition is $\mathrm{EB} \to 0$ as $\Delta/T \to \infty$. 

\begin{figure}[!htpb]
\begin{center}
\begin{subfigure}{0.8\linewidth}
    \includegraphics[width=\linewidth]{EB-4hz-6hz-lag5.png}
\end{subfigure}
\begin{subfigure}{0.8\linewidth}
    \includegraphics[width=\linewidth]{EB2-4hz-6hz.png}
\end{subfigure}
\end{center}
\caption{Top panel shows EB at f=4 $hz$ and 6 $hz$ using $\Delta$=0.017$s$. Dashed lines represent different slopes for guidance. The bottom panel shows variation in $\mathcal{EB}$, reaching an asymptotic value of 1 in the limit of $\Delta \to$ T}
\label{fig:EB}
\end{figure}

%$\mathrm{EB}$ does not appear to vanish in the limit of $\lim_{\Delta/T \to 0}$, and shows deviation from a Brownian description, d GDPs and SBMs by \citet{Metzler2015}. Also, inflection points or local extrema are found in EB which correspond to changing slopes in MSD. We observe different non-monotonic trends for $\mathrm{EB}$ depending on $f$, and overall, the magnitude is smaller for $f$=4 $\text{Hz}$ in comparison to $f$=6 $\text{Hz}$ for larger values of $\Delta$ (Figure ~\ref{fig:EB}). The length scale corresponding to diffusion as well as geometry of the confines determine the behavior of EB as the operating conditions depend on the pulsing frequency. Even though the physical confines are the same, the diffusive length scales vary based on the value of $f$. Particles in the case of $f$ = 6 $\text{Hz}$ appear to reach the boundaries faster as highlighted by the MSD plots, and we expect this to manifest in the observed EB behavior. Even after the particles have felt the effect of walls, they are influenced by spatially varying diffusivity and this results in the EB to continue increasing. This could probably be observed in the case of $f$=4 $\text{Hz}$ as well when a larger measurement window is used. It must be noted that PFB is hard-constrained in the lateral direction by walls, while gravity and hydrodynamics offer intrinsic confines in the streamwise direction.

%similar to GDP in a larger confinement \citet{Metzler2015}. Here, we posit that the length scale corresponding to diffusion as well as geometry of the confines should be considered while quantifying the behavior of EB.

In addition, we examine the spread in $\overline{\delta^{2}}$ in Figure ~\ref{fig:xi} using the non-dimensional parameter $\xi$ defined as,

\begin{equation}
    \xi = \frac{\overline{\delta^{2}(\Delta)}}{\langle \mathrm{\overline{\delta^{2}(\Delta)}} \rangle}
\end{equation}

% \noindent The width of $P(\xi)$ was observed to be greater for shorter measurement times due to smaller number of reflections from the boundaries \cite{Metzler2015}. The spread decreases when extreme excursions are impeded by boundaries. Also, the spread is greater when the confinement is larger. 

\noindent For a Brownian diffusion process, the distribution is Gaussian having a sharp peak around 1 ($\xi$ = 1 represents ergodicity). For a smaller value of $\Delta$ (10 time steps), the distribution shows a distinct peak at $\xi > 1$ and $\xi < 1$ for f=4$hz$ and 6$hz$. We notice a significant scatter in $\xi$ for growing lag times deviating from ergodic dynamics. $\phi(\xi)$ is finite at $\xi$=0 for all values of $\Delta$, which is true for sub-diffusive CTRWs \cite{Cherstvy2013}. The contribution from immobile trajectories is more prominent for longer lag times when f=4$hz$. These findings corroborate  combination of parent stochastic processes dictating the underlying anomalous diffusion. 

%There are some important differences between the two studies: (i) PFB is strongly confined in the transverse direction while the streamwise transport is effected by a weak confinement where a dynamic balance exists between drag and gravity, (ii) A particle's momentum is influenced by interaction of particles with the carrier phase as well as neighboring particles over a broad range of spatio-temporal scales. These give rise to a high degree of non-linearity possibly causing deviations from more ideal systems studied previously.

\begin{figure}[!htpb]
\begin{center}
\begin{subfigure}{0.8\linewidth}
    \includegraphics[width=\linewidth]{xi-distribution-4hz.png}
\end{subfigure}
\begin{subfigure}{0.8\linewidth}
    \includegraphics[width=\linewidth]{xi-distribution-6hz.png}
\end{subfigure}
\end{center}
\caption{Histograms of $\xi$ from experiments at f = 4$hz$ (top) and 6$hz$ (bottom).}
\label{fig:xi}
\end{figure}

Finally, we look at ageing characteristics, which along with ergodicity breaking determine the (non-)stationary nature of a stochastic process. A plot of $\langle \mathrm{\overline{\delta^{2}}} \rangle$ as a function of measurement time, T (Figure ~\ref{fig:ageing}) reveals a monotonic drop for different values of $\Delta$. This is indicative of a collective sub-diffusive anomalous process. Analogous ageing behavior in a sub-diffusive environment is found in several other systems including plasma membranes as demonstrated by \citet{Krapf2011}. The apparent diffusivity of the ensemble of particles decreases as the system evolves longer, but individual behavior could vary depending on the localized states.

\begin{figure}[!htpb]
\begin{center}
\includegraphics[width=0.8\linewidth]{ageing-4hz-6hz.png}
\end{center}
\caption{Plots of $\langle \overline{\delta^{2} \rangle}$ as a function of measurement window, T, for f = 4$hz$ (top) and 6 $hz$ (bottom).}
\label{fig:ageing}
\end{figure}

\noindent We further use ageing factor \citet{Metzler2014} defined as,
\begin{equation}
\label{eq:ageingfactor}
    \Lambda(t_{a},\Delta) = \frac{ \langle \mathrm{\overline{\delta_{a}^{2}(\Delta)}} \rangle}{\langle \mathrm{\overline{\delta^{2}(\Delta)}} \rangle}
\end{equation}

\noindent where $\overline{\delta_{a}^{2}}$ refers to the time-averaged MSD considering the ageing time $t_{a}$ given by,

\begin{equation}
\label{eq:agedmsd}
    \overline{\delta_{a}^{2}(t_{a})} =  \frac{1}{\mathrm{T}-\Delta} \int_{t_{a}}^{t_{a}+\mathrm{T}-\Delta} \langle |x_{i}(t+\Delta) - x_{i}(t)|^{2} \rangle dt
\end{equation}

\noindent The above expression is ensemble averaged while calculating $\Lambda$ for different values of ageing time shown in Figure ~\ref{fig:ageingfactor}. There is a steady drop in $\Lambda$ even for a very small value of $\Delta$. This is a consequence of continued localization of particles in static and quasi-static regions, again indicative of sub-diffusive behavior. Even though the meso-scale response of the system (based on the bubbling pattern) is completely different at f = 4$hz$ and 6$hz$, they exhibit similar anomalous diffusion characteristics.

\begin{figure}[!htpb]
\begin{center}
\includegraphics[width=0.8\linewidth]{ageingfactor-4hz-6hz.png}
\end{center}
\caption{Plots of $\Lambda$ as a function of dimensionless ageing time, $t_{a}$/T at f = 4$hz$ (top) and 6$hz$ (bottom) for different values of $\Delta$ as indicated.}
\label{fig:ageingfactor}
\end{figure}

==> sec3_Old.tex <==
%Trajectories from particle tracking are used to calculate velocity components which are normalized using,

%\begin{equation}
%\label{normalize}
%c_{i} = v_{i}/\sqrt{2v^{2}}
%\end{equation}

%\noindent where, $v_{i}$ and $v$ represent the directional velocity component and root mean square values. The histograms (Figure \ref{VDF}) confirm the existence of anisotropic and non-Maxwellian particle velocity distribution. The presence of over-populated tails is an indicator of long-range correlations in particle motion. The stream-wise velocity is slightly asymmetric. The maximum deviation from symmetry occurs around 5$\mathrm{c_{x}}$, where the excess population is due to wakes  behind bubbles which offer lesser resistance to the movement of particles. The distribution is representative of stream-wise momentum transfer in the system, in which the competing forces are interfacial drag and gravity. The deviation from a Maxwellian distribution is a result of a sequence of flight and trap events characteristic of Levy flights. Solid particles in the wake of bubbles result in transporting them over longer distances, and to maintain continuity, there is a corresponding set of particles moving in the opposite direction. This leads to over-populated tails, and their density is strongly dependent on the bubbling frequency. Non-Maxwellian VDFs have also been reported for a gravity driven granular flow \cite{Moka05} and a circulating fluidized bed \cite{AV2017}. The difference in $\mathrm{P(c_{x})}$ is not significant between 4hz and 6hz. $\mathrm{P(c_{y})}$ is symmetric due to lack of forcing in the transverse direction. However, there is a significant difference when the system is forced at 4hz and 6hz. The alternating pattern at 4hz causes particles to oscillate from side to side to displaced by the void region. The increase in forcing frequency to 6hz is accompanied by a change in the bubble pattern, hence displacing a grater population of particles.  

% \begin{figure}[!htpb]
% \begin{center}
% \begin{subfigure}{1.0\linewidth}
%     \includegraphics[width=\linewidth]{histplotx_delay5_bin0p01.png}
% \end{subfigure}
% \begin{subfigure}{1.0\linewidth}
%     \includegraphics[width=\linewidth]{histploty_delay5_bin0p01.png}
% \end{subfigure}
% \end{center}
% \caption{Distributions showing population decay over 6 decades corresponding to stream-wise (top) and transverse (bottom) motion of particles. The velocities are normalized as $c_{i} = v_{i}/\sqrt{2v^{2}}$}
% \label{VDF}
% \end{figure}

==> sec4.tex <==
We analyzed the anomalous diffusion process having a spatio-temporal dependence in PFB using single-particle tracking, and find traits from a combination of parent stochastic processes. PFB represents a weakly confined multi-particle system having complex non-linear interactions. Finite memory or long-range correlations stem from individual stochastic motions, in line with the ideas of Kac surrounding propagation of chaos \cite{Kac1956}. Time-averaged and ensemble averaged MSDs deviate indicating weak ergodicity breaking. MSDs approach a plateau similar to constrained systems for GDPs or SBMs, although the streamwise transport in PFB is effected by the balance between inter-phase drag and gravity. The distribution of amplitude scatter is wide,  non-Gaussian, asymmetric, and has a finite contribution at zero stemming from immobile particles, a feature prevalent in CTRWs. The system also exhibits ageing characteristics, which along with ergodicity breaking are suggestive of a non-stationary process. The ageing factor decreases monotonically suggesting an overall subdiffusive process at both the pulsing frequencies, which exhibit different meso-scale behavior altogether. We expect structured flow patterns while lowering the effective diffusivity compared to fluidized systems having an unperturbed inflow, which needs to be verified.
%The decay of ergodicity breaking parameter is slower compared to Brownian motion when $\Delta$/T $\to$ 0, and approaches a finite value.
